A Benchmark for Open-Domain Numerical Fact-Checking Enhanced by Claim Decomposition

Fact-checking numerical claims is critical as the presence of numbers provide mirage of veracity despite being fake potentially causing catastrophic impacts on society. The prior works in automatic fact verification do not primarily focus on natural numerical claims. A typical human fact-checker first retrieves relevant evidence addressing the different numerical aspects of the claim and then reasons about them to predict the veracity of the claim. Hence, the search process of a human fact-checker is a crucial skill that forms the foundation of the verification process. Emulating a real-world setting is essential to aid in the development of automated methods that encompass such skills. However, existing benchmarks employ heuristic claim decomposition approaches augmented with weakly supervised web search to collect evidences for verifying claims. This sometimes results in less relevant evidences and noisy sources with temporal leakage rendering a less realistic retrieval setting for claim verification. Hence, we introduce QuanTemp++: a dataset consisting of natural numerical claims, an open domain corpus, with the corresponding relevant evidence for each claim. The evidences are collected through a claim decomposition process approximately emulating the approach of human fact-checker and veracity labels ensuring there is no temporal leakage. Given this dataset, we also characterize the retrieval performance of key claim decomposition paradigms. Finally, we observe their effect on the outcome of the verification pipeline and draw insights. The code for data pipeline along with link to data can be found at https://github.com/VenkteshV/QuanTemp_Plus

==> intro_example.tex <==
\begin{table}[htb!!] % The placement specifier can be [htbp]
\centering
\scalebox{0.85}{
\begin{tcolorbox}[title= Example: Claim from \quantempplus{}] \textbf{Claim}:\texttt{Prime Minister Narendra Modi breached the \textcolor{blue}{election protocol} by addressing a rally in Howrah on \textcolor{orange}{April 6.}}


\textit{\textbf{Ideal Retrieval}}:
\begin{itemize}
    \item \ldots From cooch behar \ldots Howrah \ldots election rally on \textcolor{orange}{April 6}, pm Modi will address\ldots
    \item \ldots Election Silence Period\ldots India (\textcolor{blue}{48 to 24 hours} in advance of polling day and on polling day)\ldots 
    \item \ldots General elections were held in India in seven phases from \textcolor{brown}{11 April to 19 May 2019}\ldots
\end{itemize}
\textit{\textbf{Search Process}}:The given numerical claim requires multiple aspects to be addressed. Firstly, evidence proving that PM Modi did indeed rally on April 6 needs to be fetched. Then, the information on the election silence period and the polling schedule are to be retrieved. Given this information, the downstream verifier can then reason about the numerical aspects to form the verdict.


\end{tcolorbox}
}

\captionof{figure}{Example numerical claim from \quantempplus{}, requiring to recognize and fetch explicit and implicit evidence.}\label{intro:example} 
\end{table}%

==> table-dataset-statistics.tex <==
\begin{table*}[hbt!]
    \centering
    \small
    \begin{tabular}{p{2.9cm}
    p{2.8cm}cccccccp{0.3cm}p{0.3cm}p{0.3cm}}
    \toprule
     \textbf{Dataset}&{Complexity}& \multicolumn{1}{c}{Domain} &\multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Dev} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Corpus Size} \\
   % &\multicolumn{1}{c|}{n@10} & \multicolumn{1}{c}{RR}&\multicolumn{1}{c|}{n@10} & \multicolumn{1}{c}{RR}&\multicolumn{1}{c|}{n@10} & \multicolumn{1}{c}{RR}&\multicolumn{1}{c|}{n@10} & \multicolumn{1}{c}{RR} &\multicolumn{1}{c|}{n@10} & \multicolumn{1}{c}{RR} &\multicolumn{1}{c|}{n@10} & \multicolumn{1}{c}{RR} &\multicolumn{1}{c|}{n@10} & \multicolumn{1}{c}{RR} \\
     % & cover-EM & cover-EM& EM& EM&EM \\
     \midrule
\midrule
    \colorg \textbf{Compositional} & \colorg &  \colorg& \colorg & \colorg& \colorg& \colorg \\
MusiqueQA (2-hop) & Question& multi-domain&   14.3k&1.25k & 1.2k & 569,641 \\
     \colorg \textbf{Comp. + Compar} & \colorg & \colorg & \colorg & \colorg& \colorg&  \colorg\\
WikiMultiHopQA & Question & multi-domain  &167.5k &12.6k &12.6k & 569,641\\
StrategyQA & Question&multi-domain  &2k&221 &490 &36.6M \\
     \colorg \textbf{Disambiguation} &\colorg  &\colorg  & \colorg &\colorg &\colorg &\colorg  \\
AmbigQA &Question,Answer &multi-domain  &10k &2k & 2k&24.3M 
 & \\

     \colorg \textbf{Table+Text} &\colorg  &\colorg  & \colorg &\colorg &\colorg  & \colorg \\
OTT-QA & Evidence&multi-domain  &41.4k &2.2k &2.1k &6.5M \\
  \colorg   \textbf{Table+Text}  \colorg & \colorg  &  \colorg &  \colorg & \colorg & \colorg & \colorg  \\
  \colorg  \textbf{+Numerical} \colorg & \colorg  &  \colorg &  \colorg & \colorg & \colorg & \colorg   \\
TAT-QA &Question, Evidence & Financial   &13.2k &1.6k &1.6k &7000 \\
FinQA & Question, Evidence & Financial &6.2k &883 &1147 &24.8k \\

     \bottomrule
    \end{tabular}
    \caption{Statistics of different datasets in \name{} benchmark.}
   % \vspace{-1em}
    \label{tab:statistics}
\end{table*}
